One Snapshot is All You Need: A Generalized Method for mmWave Signal Generation

Wireless sensing systems, particularly those using mmWave technology, offer distinct advantages over traditional vision-based approaches, such as enhanced privacy and effectiveness in poor lighting conditions. These systems, leveraging FMCW signals, have shown success in human-centric applications like localization, gesture recognition, and so on. However, comprehensive mmWave datasets for diverse applications are scarce, often constrained by pre-processed signatures (e.g., point clouds or RA heatmaps) and inconsistent annotation formats. To overcome these limitations, we propose mmGen, a novel and generalized framework tailored for full-scene mmWave signal generation. By constructing physical signal transmission models, mmGen synthesizes human-reflected and environment-reflected mmWave signals from the constructed 3D meshes. Additionally, we incorporate methods to account for material properties, antenna gains, and multipath reflections, enhancing the realism of the synthesized signals. We conduct extensive experiments using a prototype system with commercial mmWave devices and Kinect sensors. The results show that the average similarity of Range-Angle and micro-Doppler signatures between the synthesized and real-captured signals across three different environments exceeds 0.91 and 0.89, respectively, demonstrating the effectiveness and practical applicability of mmGen.

==> Body/abstract.tex <==
\begin{abstract}
This paper presents a non-invasive design, namely \system, to estimate the shape and material of an object simultaneously. \system puts the object approximate to an RFID tag array, and explores the propagation effects as well as coupling effects between RFIDs and the object for sensing. 
% 
% In contrast to prior proposals, \system is capable to recognize unseen shape-material pairs as well as unseen materials within a certain container. 
In contrast to prior proposals, \system is capable to recognize unseen objects, including unseen shape-material pairs and unseen materials within a certain container.
% 
To make it real, \system introduces a sensing capability enhancement module and leverages a two-branch neural network for shape profiling and material identification respectively. Furthermore, we incorporate a Zero-Shot Learning based embedding module that incorporates the well-learned linguistic features to generalize \system to new materials. We build a prototype of \system using commodity RFID devices and comprehensive real-world experiments demonstrate our system can achieve high object estimation performance.
\end{abstract}




==> Body/discussion.tex <==
\section{Discussion and Limitation}\label{sec:discuss}
In this section, we discuss the practical issues regarding the application of \system.

\textbf{Fake material detection:}




\textbf{The number of unseen materials:} 
%





